Computational Inference in Cognitive Science: Operational, Societal and Ethical Considerations

Emerging research frontiers and computational advances have gradually transformed cognitive science into a multidisciplinary and data-driven field. As a result, there is a proliferation of cognitive theories investigated and interpreted from different academic lens and in different levels of abstraction. We formulate this applied aspect of this challenge as the computational cognitive inference, and describe the major routes of computational approaches. To balance the potential optimism alongside the speed and scale of the data-driven era of cognitive science, we propose to inspect this trend in more empirical terms by identifying the operational challenges, societal impacts and ethical guidelines in conducting research and interpreting results from the computational inference in cognitive science.

==> notes.tex <==

\item Model complexity. the simpler model.

\item Publication bias. of sample size to 

\item

\item Introduce interpretability.

Low-dimensional, highly-repeatable features: Small sample sizes will continue to be a reality of clinical applications in the near future. Models built on low-dimensional, repeatable features are more likely to generalize [19].
[19] V. Berisha, C. Krantsevich, P. R. Hahn, S. Hahn, G. Dasarathy, P. Turaga, and J. Liss, “Digital medicine and the curse of dimen- sionality,” NPJ digital medicine, vol. 4, no. 1, pp. 1–8, 2021.

Interpretable and individually-validated features: Perceptual analysis of clinical speech has a long and rich history that dates back to the 1800’s [29]. We should align our represen- tation of speech with this literature so that models can be vali- dated relative to the existing clinical knowledge base. Speech features that are individually validated are more likely to generalize across populations and clinical conditions (see next section).

Performance gap between the publications and applications 
There are al- ready several examples of ML models in healthcare that were deployed after initial evaluation on small data sets revealed good performance, only to find out that the initial performance estimates were overoptimistic [22, 23].

[23] C. Ross and I. Swetlitz, “Ibm’s watson supercomputer recom- mended ‘unsafe and incorrect’cancer treatments, internal docu- ments show,” Stat, vol. 25, 2018.
[24] A.W.EllisandA.W.Young,Humancognitiveneuropsychology: A textbook with readings. Psychology Press, 2013.

Use three levels of evaluations. 
A recently-proposed framework for validation of biomet- ric monitoring technologies provides a way forward [34]. The framework proposes three levels of evaluation: Verification of hardware, analytical Validation, and clinical Validation (V3). Verification evaluates the fidelity of the raw sample data pro- duced by the sensor technology used to acquire it in the envi- ronment in which it is to be used. Analytical validation evalu- ates the performance of the algorithms that process the raw sen- sor data to produce physiological or behavioral metrics. Clini- cal validation demonstrates that models track with a clinically- relevant ground truth or a clinically accepted measure.
Clinical speech analytics researchers tend to skip verifica- tion and analytical validation steps in favor of aiming to di- rectly evaluate the clinical validity of their model. However, we posit that this is limiting. Note that the analytical validation step is agnostic to the underlying clinical condition; rather it fo- cuses on estimating a behavioral measure of interest. For exam- ple, speaking rate and articulatory precision are impacted across many conditions [4, 35]. Having a tool that is validated at the behavior-measurement level will allow researchers to use it as a feature across many conditions for model-building. Applying this level of validation to the new pipeline proposed in the previ- ous section will result in a reusable framework for discovering and translating speech analytics across the clinical landscape.

[34]
J.C.Goldsack,A.Coravos,J.P.Bakker,B.Bent,A.V.Dowling, C. Fitzer-Attas, A. Godfrey, J. G. Godino, N. Gujar, E. Izmailova et al., “Verification, analytical validation, and clinical validation (v3): the foundation of determining fit-for-purpose for biometric monitoring technologies (biomets),” NPJ digital medicine, vol. 3, no. 1, pp. 1–15, 2020.

To machine learn or not to machine learn? Cognition is a complex construct [24]; this means that the decision bound- ary between “healthy” and “cognitively impaired” is also likely complex. Small speech databases simply don’t support the learning of such models. To compound the issue, small sample sizes make overfitting easier and increase variability, contribut- ing to the overoptimism. For small sample sizes (e.g in the tens), algorithm developers should forgo supervised learning on broad diagnostic labels for more manageable problems. For exam- ple, there is a need to develop robust speech/language features known to change with cognitive impairment (e.g. circumlocu- tion). The ground truth for these models can be attained directly from the audio and/or transcript, making it much easier to obtain than clinical labels. Furthermore, data from healthy individuals, which is much easier to obtain, can be used to augment clinical databases for development of these features, for more accurate estimates of performance, and for developing normative ranges.

The negative association between sample size and reported accuracy is seen in other machine learning studies in digital health. For example, an analysis of over 200 studies that pro- pose ML models to predict disease status from neuroimag- ing similarly showed a negative association between the re- ported accuracy and the sample size across schizophrenia, MCI, Alzheimer’s disease, major depressive disorder, and attention deficit hyperactivity disorder [18]. A similar analysis was found for classification models that predict Autism spectrum disorder using other modalities [11].
[11] A. Vabalas, E. Gowen, E. Poliakoff, and A. J. Casson, “Machine learning algorithm validation with a limited sample size,” PloS one, vol. 14, no. 11, p. e0224365, 2019.
[18] M. R. Arbabshirani, S. Plis, J. Sui, and V. D. Calhoun, “Single subject prediction of brain disorders in neuroimaging: Promises and pitfalls,” Neuroimage, vol. 145, pp. 137–165, 2017.

 More generally, repeated use of the same dataset over time - either explicitly or implicitly by relying on others that have analyzed the data previously - to improve models can lead to a similar bias [16]. 
[16] C. Dwork, V. Feldman, M. Hardt, T. Pitassi, O. Reingold, and A. Roth, “Generalization in adaptive data analysis and hold- out reuse,” Advances in Neural Information Processing Systems, vol. 28, 2015.

 It’s known that small sample size studies lead to more variable estimates of the generaliza- tion error [19]. 
 Consider multiple research labs working with a small dataset. Even if each group follows best-practices for ML model design, the small sample size will lead to a highly variable estimate of model accuracy across the groups. However, the groups with higher estimates of the accuracy are more likely to publish their model [14]. Un- der this scenario, the readers of this literature will observe the declining upper envelope of the learning curve and not its aver- age.
 [14] R.Rosenthal,“Thefiledrawerproblemandtolerancefornullre- sults.” Psychological bulletin, vol. 86, no. 3, p. 638, 1979.

Overestimation of true model accuracy in the published lit- erature provides readers with unrealistic expectations of how well these models will work once deployed; this has impor- tant downstream consequences. Model accuracy is a convenient metric for succinctly describing how well an ML model works and it’s commonly cited when the press reports on digital health. These articles raise the public’s expectations for the capabilities of ML. If these expectations aren’t met, confidence in the tech- nology and scientific literature wanes [21].
[21] S. Cave, C. Craig, K. Dihal, S. Dillon, J. Montgomery, B. Singler, and L. Taylor, “Portrayals and perceptions of ai and why they mat- ter,” 2018.
